EgoLog: Ego-Centric Fine-Grained Daily Log with Ubiquitous Wearables

Despite advances in human activity recognition (HAR) with different modalities, a precise, robust, and accurate daily log system is not yet available. Current solutions primarily rely on controlled, lab-based data collection, which limits their real-world applicability. The challenges towards a fine-grained daily log are 1) contextual awareness, 2) spatial awareness, and 3) effective fusion of multi-modal sensor data. To solve them, we propose EgoLog, which integrates effective audio-IMU fusion for daily log with ubiquitous wearables. Our approach first fuses audio and IMU data from two perspectives: temporal understanding and spatial understanding. We extract scenario-level features and aggregate them in the time dimension, while using motion compensation to enhance the performance of sound source localization. The knowledge obtained from these steps is then integrated into a multi-modal HAR framework. Here, the scenario provides prior knowledge, and the spatial location helps differentiate the user from the background. Furthermore, we integrate a LLM to enhance scenario recognition through logical reasoning. The knowledge derived from the LLM is subsequently transferred back to the local device to enable efficient, on-device inference. Evaluated on both public and self-collected dataset, EgoLog achieves effective multimodal fusion for both activity and scenraio recognition, outperforms the baseline by 12% and 15%, respectively.

==> response/responseA.tex <==
\vspace{-1em}
\subsection{Response to Reviewer A}
\setcounter{reviewcounter}{1}

\begin{review}
Motivation and practicality. The motivation for using earable sensors as the primary platform for daily life logging is not well supported. Earable devices typically suffer from limited battery life, making continuous streaming of audio and IMU data to a smartphone impractical. Additionally, users do not wear earbuds throughout the day; earbuds are often used only during work or specific activities. These factors make earables a less suitable platform for comprehensive daily life logging. A more natural target device might be smart glasses, which are more consistently worn in free-living environments.
\end{review}

\begin{response}
We thank the reviewer for highlighting the practical limitations of earables for daily life logging. In response, we have expanded the target platforms of \systemname{} to include not only earables but also smart glasses, smartwatches, and smartphones. This multi-platform approach significantly enhances the practicality and broadens the potential user base of our system. We agree that smart glasses, which are more consistently worn in free-living environments, are a more natural and suitable platform for comprehensive daily logging. \newresponse{The experiment (Sec. 5) and introduction (Sec. 1) have been updated to reflect this broader scope, with evaluations conducted across the different device types.}
\end{response}

\begin{review}
Limited novelty. The proposed solution largely builds on existing techniques. Contextual understanding via contrastive learning and sound source localization with binaural audio have both been widely studied in prior work. The main potential contribution appears to be in Sec. 4.4, where contextual fusion is discussed; however, the authors rely directly on ImageBind without introducing new architectural designs or fusion mechanisms.
\end{review}

\begin{response}
\newresponse{We have reorganized our contributions and added new designs to enhance the technical depth of our work in Sec. 4.} Specifically, we propose a novel audio-IMU fusion method 
for fine-grained ego-centric activity recognition that considers both temporal and spatial understanding. We extract the scenario-level features through contrastive learning, which differs from conventional end-to-end learning and benefits the scenario recognition. Additionally, we develop an adaptive calibration method with sound source localization and motion data to resolve issues such as front–back confusion. 

As noted by the reviewer, we propose a new HAR method for ego-centric sensing that can innovatively understand the scenario and the environment.
To achieve this, we leverage two aspects of information: On one hand, we distinguish similar activities by leveraging the extracted scenario information. On the other hand, we use the sound source and audio-IMU correlation to differentiate the user-generated sounds from background sounds.

Finally, in the updated Sec. 4.5, we propose an LLM-assisted scenario recognition paradigm. In this framework, processed sensor data is fed into an LLM for high-level reasoning. The LLM's output is then used to transfer actionable knowledge back to the local device for on-device inference.

\end{response}

\begin{review}
Unclear methodology for HAR. It is unclear how the authors achieve the final human activity recognition step. While Sec. 4.4 describes multi-modal fusion, there is little detail on how the recognition model itself is trained or whether any specialized training strategies were developed for this purpose.
\end{review}

\begin{response}
\newresponse{
The writing of Sec. 4.4 has been refined to provide a clearer illustration of our design.
} 
Specifically, the scenario description obtained from Sec. \ref{sec:scenario} is processed by the text encoder from ImageBind. The resulting embedding is then fused with features from the audio and IMU encoders, which are lightweight.
The multi-modal fusion is performed using cross-modal attention, where the scenario embedding is treated as one of the input modalities. For the training objective, we employ a standard cross-entropy loss for this classification task.

\end{response}

\begin{review}
Limited activity set. The evaluation is conducted on only about 20 activities, which represent a very small and coarse-grained subset of daily life activities. Many HAR studies evaluate hundreds of activities, and the limited coverage here raises questions about the system’s ability to generalize. It is unclear how the system would handle activities outside the predefined set.
\end{review}

\begin{response}
We thank the reviewer for pointing out this limitation. In the current submission, \newresponse{both the public dataset and the self-collected dataset are updated in Sec. 5.} 
Our public datasets include Ego4D, EgoADL, and SAMOSA, which feature extensive activity sets up to hundreds of activities in diverse scenarios (91), where we validate our approach.
On the other hand, we acknowledge that our resources are not comparable to Ego4D and also not necessary to re-collect a large-scale dataset with no difference. Therefore, the focus of our dataset is to validate spatial understanding, an aspect that is lacking in other public datasets. As the reviewer suggested, we have also enriched the activity set of our own dataset as much as possible.
\end{response}

\begin{review}
Unfair comparison with baseline. The baselines chosen for comparison are not specifically designed or trained for HAR tasks. This makes the comparative evaluation less convincing. It is also unclear whether the baselines were provided with the predefined HAR classes, which may bias the results.
\end{review}

\begin{response}
In our revised paper, \newresponse{we have updated the baselines for both activity and scenario recognition with detailed descriptions in Sec. 5}. For activity recognition, the baselines are SAMOSA and ImageBind-FT, both trained on the same set of predefined HAR classes. For scenario recognition, we also consider SAMOSA and ImageBind-FT, and we have added Qwen-Audio as a strong generative baseline that is not constrained by predefined classes.
\end{response}



==> response/responseB.tex <==
\vspace{-1em}
\subsection{Response to Reviewer B}
\setcounter{reviewcounter}{1}

\begin{review}
The paper assumes that incorporating contextual and spatial priors into a transformer fusion module enables better activity recognition, but does not analyze how or why fusion improves performance for specific activity types. A visualization of attention maps or modality contribution (e.g., SHAP, saliency) would help justify the architecture.

\end{review}

\begin{response}
\newresponse{The motivation study in Sec. \ref{sec:measurement} is refined to justify the reasoning of using those priors.}
Specifically, we explain why the scenario (contextual prior) helps with HAR in Figure 2, where we observe that activities within the same scenario exhibit higher similarity. The benefit of using this prior is further demonstrated in the evaluation.
For the spatial prior, which helps differentiate between foreground and background, we illustrate in Sec. 3 that a simple volume-based approach is insufficient, making sound source localization necessary. 
\end{response}

\begin{review}
While ROUGE scores are reported, summary quality is not analyzed qualitatively or through a human study. Without measuring hallucination, factual correctness, or usefulness, it is hard to evaluate how meaningful the summaries are.
\end{review}

\begin{response}
Thank you for your feedback. In the revised paper, we have included both subjective and objective evaluations. The subjective evaluation is based on a user study that incorporates the specific dimension suggested by the reviewer
\end{response}

\begin{review}
The runtime breakdown suggests the system is relatively lightweight, but many components (e.g., binaural STFT + separation + fusion) remain non-trivial. A more explicit discussion of deployment modes (e.g., periodic summary vs. real-time logging) and trade-offs would improve practical clarity.
\end{review}

\begin{response}
\newresponse{We have updated our system design to better support lightweight deployment, mainly in Sec. 4.2.} Specifically, we have replaced the ImageBind model with a smaller alternative. We also made the separation module optional, as it is less critical to our design. Consequently, the remaining modules are all lightweight, with the exception of the LLM. The LLM is only called infrequently, and we discuss the frequency of its calls in the paper.
\end{response}

\begin{review}
Sound localization is subject to HRTF variability across users. While Fig. 21 shows per-user accuracy, there is no discussion of model personalization or adaptation techniques.
\end{review}

\begin{response}
The per-user performance in Fig. 26 indicates that cross-user variance is not significant. In Sec. 6, we discuss future work on unsupervised learning to eliminate the need for data collection. It is also worth noting that the updated \systemname{} supports other devices besides earphones. Since these devices do not rely on user-specific HRTFs, they are not subject to this limitation.
\end{response}

\begin{review}
While the proposed contrastive learning-based alignment of audio and IMU embeddings is well-motivated, the paper does not benchmark this approach against other established or alternative alignment techniques.

\end{review}

\begin{response}
We thank the reviewer for this suggestion. To address this, we have added a comparison with ImageBind-FT as a strong baseline. ImageBind is pre-trained to align various modalities (e.g., audio-image, IMU-image) through a shared image embedding space. By fine-tuning it (ImageBind-FT) on our task, we can provide a fair comparison that highlights the advantages of our proposed contrastive alignment method between audio and IMU modalities.
\end{response}



==> response/responseC.tex <==
\vspace{-1em}
\subsection{Response to Reviewer C}
\setcounter{reviewcounter}{1}

\begin{review}
The individual components, such as contrastive learning-based multimodal feature extraction or ImageBind for multimodal fusion, are based on existing approaches and not necessarily novel. The rationale for choosing these approaches over other established alternatives is not clear.

\end{review}

\begin{response}
In the revised version of our paper, we have updated the rationale in each subsection of Section 4, as well as in the corresponding paragraph of the measurement study.

Regarding the reviewer's question, we would like to highlight that we are the first to apply contrastive learning to audio-IMU data, with the goal of extracting scenario-level features. Unlike other contrastive learning methods that aim for one modality to retrieve the other, our objective is different: we seek to find similarities between the two modalities, which are highly relevant to the scenario in a long-term manner.
As for ImageBind, we only use its text encoder to encode scenario descriptions (text) into our novel human activity recognition (HAR) framework, as described in Section \ref{sec:har}.

\end{response}

\begin{review}
While using LLMs to generate egocentric summaries of activity is interesting, there is no evaluation of the utility of such summaries from a user perspective.
\end{review}

\begin{response}
\newresponse{In this revision, we have extended LLM's role into scenario refinement in Sec. 4.4}. Specifically, the audio and IMU data are processed into text, along with the scenario and spatial information, to serve as input to the LLM. The LLM then performs reasoning to estimate the scenario, leveraging its inherent advantages for such tasks.
Correspondingly, to evaluate this enhanced component comprehensively, we have provided a detailed evaluation in the form of scenario recognition. Additionally, we have updated the user study to focus specifically on participants' subjective experiences rather than on evaluating the LLM itself.
\end{response}

\begin{review}
For Summary Generation, how were the five scenario clusters selected for evaluation? What are the different LLMs used for evaluation?
\end{review}

\begin{response}
In our revised paper, the LLM component is designed to be generalizable across all scenarios, allowing it to fully utilize its reasoning capabilities.
\end{response}

\begin{review}
For HAR, the authors report that performance drops when using 1-second windows but the exact metrics are not available in Fig 14. Also, what is the "All" duration in this figure?

Report means and SDs for analyses across different activities (Fig 15), scenarios (Fig 22), and users (Fig 21).
\end{review}

\begin{response}
In our revised paper, Fig. 18 is updated to show the performance of HAR with different data length, from 2 seconds to 10 seconds. We also present some number in the description.
On the other hand, we also update most of the figures.
\end{response}


\begin{review}
Using secondary annotations (from [10, 11]) for the HAR model when binaural audio is not available might impact the overall performance and should be discussed.
\end{review}

\begin{response}
In our revised paper, \newresponse{the evaluation of spatial understanding is primarily conducted using our self-collected dataset in Sec. 5}, which features high-precision annotations.
\end{response}

\begin{review}
The insights from the Motivation Study are mostly well-known, so Sec. 3 can be more brief.
\end{review}

\begin{response}
\newresponse{We have revised Sec. \ref{sec:measurement} to be more concise and polish the content.}
Specifically, we fully rewrite the part of sound localization, motivating the need for motion compensation. Besides, we refine the other content by keeping it concise and removing the well-known things.
\end{response}

\begin{review}
The paper can be improved in terms of the terminology used (e.g., "scenario" vs "context" are sometimes used interchangeably, terms can be defined more clearly in the Introduction) and organization (some figures are out of order, e.g., Fig 17 and 18).

\end{review}

\begin{response}
We thank the reviewer for this important point. We have now clearly differentiated the terms "scenario" and "context" throughout the paper.
Specifically, "scenario" is the most frequently used term, representing the high-level, long-term activity label, which is also the target of our design. In contrast, "context" is treated as a more general concept. For example, our design goal is to extract contextual information in the form of a scenario, and all the information fed to the LLM is also considered context.
\end{response}

\begin{review}
The framework diagrams (Fig 7 through 9) can be clearer. E.g., it's not clear how the outputs of the first two blocks are integrated in the Contextual Fusion for HAR in Fig 7, although this is explained in Sec 4.4.
\end{review}

\begin{response}
\newresponse{The framework diagrams (system overview) are updated in the revised paper.}
\end{response}




==> response/responseD.tex <==
\vspace{-1em}
\subsection{Response to Reviewer D}
\setcounter{reviewcounter}{1}

\begin{review}
I think the method of incorporating the scenario and spatial information is described at a very high level. How exactly is the scenario information structured and fed into the transformer? How is the "trigger" for near-field vs. far-field implemented technically during model inference? Please provide more details for the algorithm.
\end{review}

\begin{response}
\newresponse{
In our revised paper, we have significantly updated the method for incorporating scenario and spatial information in Sec. \ref{sec:har} and \ref{sec:llm}.
}
\begin{itemize}
    \item We represent scenario information as a text embedding and integrate it via a self-attention mechanism to enhance activity recognition. For LLM-based reasoning, we incorporate the scenario through corresponding prompts, using initial recognition results as input to improve reasoning performance.
    
    \item We process spatial information differently for near-field and far-field scenarios. For activity recognition, we disable audio processing and revert to motion sensing when far-field sound is detected (by confidence), reducing interference. For LLM-based scenario recognition, both near-field and far-field inputs are retained but processed with different prompts, as both contribute to scenario understanding.
\end{itemize}

\end{response}

\begin{review}
It is not clear that how the sound localization and separation module is utilized in the final HAR pipeline. More details are needed.
\end{review}

\begin{response}
In our revised paper, \newresponse{we have refined the role of the sound localization module in Sec. 4.2}. Its function is now more prominent in the new "LLM-based scenario refinement" subsection, where sounds are classified as near-field or far-field to provide spatial context for the LLM. Conversely, we have opted to omit the sound separation module. As this component is computationally expensive and was found to be non-essential for the LLM's reasoning process, its inclusion was deemed unnecessary.
\end{response}

\begin{review}
The paper claims to "distinguish near-field and far-field audio sources" but the evaluation in Fig. 17 only shows accuracy for localizing a single source. The much harder and more realistic problem of separating a mixture of sources (e.g., user's voice + far-field music) is not evaluated for its impact on HAR performance.
\end{review}

\begin{response}
In our revised paper, \newresponse{we have expanded our self-collected dataset to include more diverse scenarios in Sec. 5}, particularly those with multiple sound sources. Our evaluation now focuses on two key aspects: the performance of the sound localization module itself, and its impact on downstream tasks, such as LLM-based reasoning.
\end{response}

\begin{review}
The "Key Frame" Concept is Confusing: In Sec. 4.2.2, the concept of "key frames" (samples with high audio-IMU similarity) is introduced. However, it's unclear how these are selected in practice during inference. What is the threshold for "high similarity"? Is this a hyperparameter? How often do these key frames occur? The reliance on a sparse, undefined signal adds uncertainty to the scenario recognition pipeline.
\end{review}

\begin{response}
In our revised manuscript, we have refined this process to eliminate the ambiguity discussed in Sec. \ref{sec:scenario}. Instead of relying on a dynamic similarity threshold during inference, we now employ a static sequence model after contrastive learning.
The embeddings from each modality are concatenated along the channel dimension and then fed into the model. Although the features remain sparse due to their content, our sequence model can automatically identify the "key frames" and ignore the others.

\end{response}

\begin{review}
Even though the authors consider multiple different environments in Sec. 5.4 (sound localization performance), the details of the environments are missing. Do the environments involve different noise or dynamic interference? It is not clear how the system handles highly dynamic or noisy environments. User movement, background noise, and interaction with the environment may affect the accuracy of both spatial audio localization and activity recognition.

\end{review}
\begin{response}
\newresponse{In our revised paper, the details and diversity of the self-collected dataset are elaborated and improved}. Please see the update on the paper.
\end{response}

\begin{review}
It would be great if the authors can add more details to sufficiently explain how the combination of contrastive learning, key frame selection, and temporal aggregation overcomes the inherent weak correlation between audio and IMU data.
\end{review}

\begin{response}
\newresponse{
We have updated both the design in Sec. \ref{sec:scenario} and ablation study in Sec. \ref{sec:evaluation} to resolve the reviewer's concern.
}
Specifically, the contrastive learning forces the two modalities to project to the same feature space, even though their correlation is weak. We consider the frame with high correlation as a key frame, while the others as relatively useless. To effectively utilize all of them, we perform temporal aggregation in the form of a sequence model. The updated ablation study confirms the necessity of each component.
\end{response}

\begin{review}
The sensing module seems output only one activity label at a time, whereas real-life activities are often concurrent (e.g., walking while talking on the phone). Even sequential outputs such as “walking” followed by “talking on the phone” may degrade the quality of the generated daily log.
\end{review}

\begin{response}
We acknowledge the problem raised by the reviewer. This issue can be alleviated by using a sliding window approach. We also considered incorporating multi-label classification; however, annotating and collecting such a dataset is extremely challenging.
Although the above design does not completely solve the problem, we would like to emphasize that the daily log remains robust despite such perturbations. Specifically, we present the log in the form of scenarios and histograms of activities. The former is compatible with multi-label outputs, while the latter provides a statistical summary. \newresponse{We demonstrate in Section 5 that these types of outputs meet users' needs.}
\end{response}


==> response/responseE.tex <==
\vspace{-1em}
\subsection{Response to Reviewer E}
\setcounter{reviewcounter}{1}

\begin{review}
This is an interesting work and has a nice motivation on logging context and activities. The system design seems sound, but is mostly focused on integrating existing techniques (including the LLM aspect at the end?). In one sense, the integration to make a complete product is quite nice, however, the evaluation results and scores are not as high, even for what appears to be a carefully curated dataset with only a few activities. Of course, questions around the generalization of the technique remain in that sense.


\end{review}

\begin{response}
We reformulate our technical novelty below:
\begin{itemize}
    \item We employ multi-modal fusion to enhance temporal and spatial understanding, rather than performing direct human activity recognition. Temporal understanding involves recognizing the long-term scenario, while spatial understanding utilizes motion data to compensate for sound source localization. Both aspects are crucial for subsequent processing stages.
    
    \item In response to the reviewer's interest in Sec. \ref{sec:har}, we have refined it to better highlight our novelty: the incorporation of previously extracted scenario information alongside raw data, based on the ImageBind model.
    
    \item Furthermore, the initial user study on using an LLM for summarization has been expanded into a formal design. In this design, we utilize an LLM to recognize the scenario and then transfer this knowledge back to the local device.

\end{itemize}

Regarding the evaluation results, our recognition performance is relatively modest due to the high diversity of the Ego4D dataset. However, the accuracy reaches 60\%when the number of classes is clustered to five.
More importantly, we combine activity and scenario recognition into a daily log. The scenario recognition component exhibits about 80\%accuracy. Although the activity results are presented in a histogram format, they are still considered useful according to our user study.

Lastly, although our design is mainly close-set classification, the LLM-based scenario recognition has potential for better generalization, and \newresponse{we include a discussion for it in Sec. \ref{sec:discussion}.}

\end{response}




==> response/response_main.tex <==
\textbf{Previous submission: \#50 EarLog: Enabling Egocentric Acoustic Sensing for Daily Log with Earables.}
We sincerely thank the reviewers of the previous submission of SenSys'26 for their time and valuable feedback, which has been instrumental in helping us improve our paper. 
We have revised the title to better reflect the scope of the paper, as our target platforms are not limited to earphones. In accordance with the reviewer's suggestion, we clarify that \systemname{} is applicable to any wearable device equipped with both audio and IMU sensing capabilities. Furthermore, we have explicitly defined "daily log" as our primary target, which encompasses both activity and scenario recognition.

This document outlines our response to the reviewers. Following the SenSys Call for Papers guidelines, we first provide a summary of the main improvements, followed by point-by-point responses to each comment.
In the revised manuscript, we use blue text to highlight the modifications made to the paper, both in the manuscript and in the response below.

\section{Revision Summary}
\begin{itemize}
    \item 
    \textbf{(RA-C1):}
    \newresponse{We have comprehensively revised the paper. The introduction and overall design goal have been refined to better highlight the practicality.}
    In the current manuscript, \systemname{} is designed for both activity recognition and scenario recognition, which represent the user's daily log. Our system can be implemented on ubiquitous wearables, not limited to earphones, as long as they possess audio and IMU sensing capabilities. Unlike previous studies on HAR that are confined to lab-collected datasets, \systemname{} is designed to be context-aware and environment-aware, making it much closer to real-world conditions.

    \item
    \textbf{(RA-C2,3\&RC-C1\&RD-C1,4):}
    \newresponse{The system design and corresponding figures have been updated to illustrate our technical novelty.} Sec. \ref{sec:scenario} has been renamed to ``Temporal Understanding'' to reduce ambiguity between the terms context and scenario, and details, particularly regarding key frame selection, have been updated. Sec. \ref{sec:localization} has been polished with additional details, and its corresponding motivation section has also been refined. Sec. \ref{sec:har} has been improved with clearer explanations.
    
    \item
    \textbf{(RB-C2\&RC-C2\&RE-C1)}
    \newresponse{An extension of the previous user study (using LLM for summary) as part of the system design}. 
    In our previous submission, we used an LLM to generate summaries. We found that these summaries were closely related to the scenario, indicating that an LLM can perform scenario recognition with strong generalization. However, due to the high computational cost of LLMs, which makes them unsuitable for local deployment, a key challenge is how to effectively collaborate an LLM with a local, lightweight model.

    \item 
    \textbf{(RB-C1\&RC-C6\&RD-C3)}
    \newresponse{We have significantly improved the motivation study in Sec. \ref{sec:measurement}}. 
    The revisions include an enriched explanation of spatial understanding, which demonstrates how user motion refines sound localization and enables near-far audio classification. This classification is central to differentiating the user's activities from those of others.
    
    \item 
    \textbf{(RA-C4\&RD-C6)}
    \newresponse{We provided new experiments to validate \systemname{} in Sec. \ref{sec:evaluation}}. The public datasets cover various devices, including smart glasses, smartwatch and smartphones. For our self-collected dataset, we also collect it with different devices to validate our design (specifically for the spatial understanding). For the updated design, the corresponding ablation study and micro-benchmark are updated.

\end{itemize}

\vspace{-1em}
\section{Detailed Responses}
\setcounter{reviewcounter}{1}

\begin{review}
    TPC Summary: This paper was discussed both online and during the TPC meeting. The overall consensus is that it presents an interesting idea and is well-written as a system paper, but its novelty is limited, with unclear methodological details and evaluation gaps. Reviewers specifically noted limited technical contributions to the existing methods, like multimodal framework and binaural sound localization, as well as concerns about the small and coarse-grained activity set, generalization to real-world scenarios, and potentially unfair baseline comparisons. We encourage the authors to address these issues and consider resubmitting in a future cycle.
\end{review}

\begin{response}
All reviewer concerns have been addressed. Our detailed responses are provided below, adhering to the page limit constraints.
\end{response}

\input{response/responseA}
\input{response/responseB}
\input{response/responseC}
\input{response/responseD}
\input{response/responseE}




